Single Stage DOA-Frequency Representation of the Array Data with Source Reconstruction Capability

In this paper, a new signal processing framework is proposed, in which the array time samples are represented in DOA-frequency domain through a single stage problem. It is shown that concatenated array data is well represented in a $\mathbf{G}$ dictionary atoms space, where $\mathbf{G}$ columns correspond to pixels in the DOA-frequency image. We present two approaches for the $\mathbf{G}$ formation and compare the benefits and disadvantages of them. A mutual coherence guaranteed $\mathbf{G}$ manipulation technique is also proposed. Furthermore, unlike most of the existing methods, the proposed problem is reversible into the time domain, therefore, source recovery from the resulted DOA-frequency image is possible. The proposed representation in DOA-frequency domain can be simply transformed into a group sparse problem, in the case of non-multitone sources in a given bandwidth. Therefore, it can also be utilized as an effective wideband DOA estimator. In the simulation part, two scenarios of multitone sources with unknown frequency and DOA locations and non-multitone wideband sources with assumed frequency region are examined. In multitone scenario, sparse solvers yield more accurate DOA-frequency representation compared to some noncoherent approaches. At the latter scenario, the proposed method with group sparse solver outperforms some existing wideband DOA estimators in low SNR regime. In addition, sources' recovery simultaneous with DOA estimation shows significant improvement compared to the conventional delay and sum beamformer and without prerequisites required in sophisticated wideband beamformers.

==> src/file3_Wid.tex <==
\section{Solutions for wideband sources}
issues such as focusing matrices and l1-svd\cite{malioutov2005sparse} comes here.

To deal with this issue, a common approach is to split signal into multiple narrowband regions by using a filter bank or Discrete Fourier Transform (DFT) and then applying the narrowband methods for each frequency sub-band. This approach is almost unique solution proposed in many old and recent researches \cite{Wang1985,DiClaudio2001,Hyder2010,Yoon2006a,malioutov2005sparse}.
$\ell_0$
